Pattern-Selective Feedback Stabilization of Ginzburg--Landau Spiral Waves

The complex Ginzburg--Landau equation serves as a paradigm of pattern formation and the existence and stability properties of Ginzburg--Landau $m$-armed spiral waves have been investigated extensively. However, many multi-armed spiral waves are unstable and thereby rarely visible in experiments and numerical simulations. In this article we selectively stabilize certain significant classes of unstable spiral waves within circular and spherical geometries. As a result, stable spiral waves with an arbitrary number of arms are obtained for the first time. Our tool for stabilization is the symmetry-breaking control triple method, which is an equivariant generalization of the widely applied Pyragas control to the setting of PDEs.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{ArKr02} I. Aranson and L. Kramer. The world of the complex Ginzburg--Landau equation. \textit{Rev. Modern Phys.} \textbf{74}, 99--143, (2002).

\bibitem{ChLa00} P. Chossat and R. Lauterbach. \textit{Methods in Equivariant Bifurcations and Dynamical Systems}. World Scientific Publishing Co. Pte. Ltd, (2000).

\bibitem{DaRong20} D. R. Cheng. Instability of solutions to the Ginzburg–Landau equation on $\mathbb{S}^n$ and $\mathbb{CP}^n$. \textit{Journal of Functional Analysis}, \textbf{Vol. 279}, 108669, (2020).

\bibitem{Da20} J.-Y. Dai. Ginzburg--Landau Spiral Waves in Circular and Spherical Geometries. \textit{SIAM Journal on Mathematical Analysis}, \textbf{Vol. 53}, 1004--1028, (2021).

\bibitem{DaLa21} J.-Y. Dai and P. Lappicy. Ginzburg--Landau patterns in circular and spherical geometries: vortices, spirals, and attractors. \textit{SIAM Journal on Applied Dynamical Systems}, \textbf{Vol. 20}, 1959--1984, (2021).

\bibitem{Duetal92} Q. Du, M. G. Max. and J. S. Peterson. Analysis and Approximation of the {G}inzburg–{L}andau Model of Superconductivity. \textit{SIAM Review} \textbf{34}, 54--81, (1992).

\bibitem{FiSc03} 
B. Fiedler and A. Scheel. 
Spatio-Temporal Dynamics of Reaction-Diffusion Patterns. 
\textit{Trends in Nonlinear Analysis}, Springer-Verlag Berlin Heidelberg, 23--152, (2003). 

\bibitem{FIE20}
B. Fiedler and I. Schneider.
Stabilized rapid oscillations in a delay equation: Feedback control by a small resonant delay.
\textit{Discrete and Continuous Dynamical Systems - Series S}, \textbf{Vol. 13}, (2020).

\bibitem{GoSt03} M. Golubitsky and I. Stewart. \textit{The Symmetry Perspective}. Birkh\"{a}user-Verlag, (2003).

\bibitem{Ha82} P. S. Hagen. Spiral Waves in Reaction-Diffusion Equations. \textit{SIAM Journal on Applied Mathematics}, \textbf{42}, 762--786, (1982).

\bibitem{He81} D. Henry. \textit{Geometric theory of semilinear parabolic equations}. Springer-Verlag Berlin Heidelberg (1981).

\bibitem{HOE05} P. H{\"o}vel and E. Sch{\"o}ll. Control of unstable steady states by time-delayed feedback methods. \textit{Physical Review E} \textbf{72}, 046203, (2005).

\bibitem{Ka95} T. Kato. \textit{Perturbation Theory for Linear Operators}. Springer-Verlag Berlin Heidelberg (1995).

\bibitem{KHE02}O.-U. Kheowan, V. S. Zykov, and S. C.  M{\"u}ller. Transition from local to global feedback control of spiral wave dynamics.
\textit{Physical Chemistry Chemical Physics} \textbf{4}, 1334--1338, (2002).

\bibitem{KIM01}
M. Kim, M. Bertram, M. Pollmann, M., A. V. Oertzen, A. S. Mikhailov, H. H. Rotermund, and G. Ertl. Controlling chemical turbulence by global delayed feedback: pattern formation in catalytic CO oxidation on Pt(110). \textit{Science}, \textbf{292}(5520), 1357--1360, (2001).

\bibitem{KoHo81} N. Kopell and L. N. Howard. Target pattern and spiral solutions to reaction-diffusion equations with more than one space dimension. \textit{Adv. App. Math.} \textbf{2}, 417--449, (1981).

\bibitem{LEK95} A. Lekebusch, A. F{\"o}rster, and F. W. Schneider. Chaos control in an enzymatic reaction. \textit{Journal of Physical Chemistry} \textbf{99}, 681--686, (1995).

\bibitem{LU96} W. Lu, D. Yu, and R. G. Harrison. Control of patterns in spatiotemporal chaos in optics. \textit{Physical Review Letters} \textbf{76}, 3316, (1996).

\bibitem{Mi05} P. Mironescu. On the Stability of Radial Solutions of the Ginzburg--Landau Equation. \textit{Journal of Functional Analysis}, \textbf{Vol. 130}, 334--344, (1995).

\bibitem{MON04} K. A. Montgomery and M. Silber. Feedback control of travelling wave solutions of the complex Ginzburg–Landau equation. \textit{Nonlinearity} \textbf{17}, 2225, (2004).

\bibitem{Mu03} J. D. Murray. \textit{Mathematical Biology II: Spatial Models and Biomedical Applications}. Springer-Verlag New York, (2003).

\bibitem{OMA12} H. M. Omar. \textit{Control optimization method for helicopters carrying suspended loads}. US Patent 8190307B2, (2012).

\bibitem{PAN00}
A. V. Panfilov, S. C.Müller, V. S. Zykov, and  J. P. Keener. Elimination of spiral waves in cardiac tissue by multiple electrical shocks. \textit{Physical Review E}, \textbf{61}(4), 4644, (2000).

\bibitem{Pi99} L. M. Pismen. \textit{Vortices in Nonlinear Fields: From Liquid Crystals to Superfluids, from Non-equilibrium Patterns to Cosmic Strings}. Clarendon Press, (1999).

\bibitem{POS07} C. M. Postlethwaite and M. Silber. Spatial and temporal feedback control of traveling wave solutions of the two-dimensional complex Ginzburg–Landau equation. \textit{Physica D: Nonlinear Phenomena} \textbf{236}, 65--74, (2007).

\bibitem{PYR92}K. Pyragas. Continuous control of chaos by self-controlling feedback. \textit{Physics Letters A}, \textbf{170}, 421--428, (1992).

\bibitem{SaSc20} B. Sandstede and A. Scheel. Spiral waves: Linear and nonlinear theory. \textit{To appear in Memoirs Amer. Math. Soc.}, \href{https://arxiv.org/abs/2002.10352}{arXiv:2002.10352}, (2020).

\bibitem{SCH06} S. Schikora, P. H{\"o}vel, H-J W{\"u}nsche, E. Sch{\"o}ll, and F. Henneberger. All-optical noninvasive control of unstable steady states in a semiconductor laser. \textit{Physical Review Letters} \textbf{97}, 213902, (2006).

\bibitem{SCH93} F. W. Schneider, R. Blittersdorf, A. F{\"o}rster, T. Hauck, D. Lebender, and J. M{\"u}ller. Continuous control of chemical chaos by time delayed feedback. \textit{Journal of Physical Chemistry} \textbf{97}, 12244--12248, (1993).

\bibitem{Sch16a} I. Schneider and M. Bosewitz. Eliminating restrictions of time-delayed feedback control using equivariance. \textit{Discrete and Continuous Dynamical Systems A} \textbf{36}, 451, (2016).

\bibitem{Sch16} I. Schneider. \textit{Spatio-Temporal Feedback Control of Partial Differential Equations}. Ph.D. thesis, Freie Universit\"{a}t Berlin, (2016).

\bibitem{Sch18} I. Schneider, An Introduction to the Control Triple Method for Partial Differential Equations. \textit{Patterns of Dynamics}. Springer, 269--285, (2018).

\bibitem{Se05} S. Serfaty. Stability in 2D Ginzburg--Landau passes to the limit. \textit{Indiana Univ. Math. J.} \textbf{54(1)}, 199--222, (2005).

\bibitem{Sm11} H. Smith. \textit{An Introduction to Delay Differential Equations with Applications to the Life Sciences}, Springer, (2011).

\bibitem{TOT18}
J.F. Totz, J. Rode, M.R. Tinsley, K. Showalter, and H. Engel,
Spiral wave chimera states in large populations of coupled chemical oscillators,
\textit{Nature Physics},
\textbf{14}, 282--285 (2018).

\bibitem{VAN00} V. K. Vanag, L. Yang, M. Dolnik, A. M. Zhabotinsky, and I. R. Epstein. Oscillatory cluster patterns in a homogeneous chemical system with global feedback. \textit{Nature}, \textbf{406}(6794), 389--391, (2000).

\bibitem{Va82}
A.~Vanderbauwhede.
\emph {Local Bifurcation and Symmetry}.
Research Notes in Mathematics, (1982).

\bibitem{proefschrift}
B. de Wolff. 
\emph{Delayed feedback stabilization with and without symmetry}. Ph.D. thesis, Freie Universit{\"a}t Berlin, (2021). 

\bibitem{oddnumber}
B. de Wolff and I.  Schneider, 
Geometric invariance of determining and resonating centers: Odd- and any-number limitations of Pyragas control, \textit{Chaos} \textbf{31}, 6, (2021). 


\bibitem{Wu96} J. Wu. \textit{Theory and Applications of Partial Functional Differential Equations}. \textbf{Vol. 119}, Applied Mathematical Sciences, Springer, (1996).

\bibitem{YAM09} K. Yamasue, K. Kobayashi, H. Yamada, K. Matsushige, and T. Hikihara. Controlling chaos in dynamic-mode atomic force microscope. \textit{Physics Letters A} \textbf{373}, 3140--3144, (2009).

\end{thebibliography}


